A Unified Model of Text and Citations for Topic-Specific Citation Networks

Social scientists analyze citation networks to study how documents influence subsequent work across various domains such as judicial politics and international relations. However, conventional approaches that summarize document attributes in citation networks often overlook the diverse semantic contexts in which citations occur. This paper develops the paragraph-citation topic model (PCTM), which analyzes citation networks and document texts jointly. The PCTM extends conventional topic models by assigning topics to paragraphs of citing documents, allowing citations to share topics with their embedding paragraphs. Our empirical analysis of U.S. Supreme Court opinions in the privacy issue domain, which includes cases on reproductive rights, demonstrates that citations within individual documents frequently span multiple substantive areas, and citations to individual documents show considerable topical diversity.

==> inputs/prediction.tex <==
\section{Posterior Predictive Distributions of PCTM}

$\mathbf{W}_{iq}$ is a vector of length $n_{iq}$, the number of words in paragraph $q$ of document $i$, and its $l$ th element, $W_{iql}$, is the $l$ the word in paragraph $p$ of document $i$.
$\mathbf{D}_{iq}$ is a vector of length $i-1$, the number of all possible documents to be cited, and its $j$ th element, $D_{iqj}$ is 1 if paragraph $p$ of document $i$ cited document $j$; 0 otherwise.
We use $\mathbf{W}_{iq}$ and $\mathbf{D}_{iq}$ as the test data to be predicted, and all words and citations in other paragraph than $q$ in document $i$ as well as all data in previous documents as the training data.
Thus, $\mathbf{W}^{train}$ be the set of $\mathbf{W}_{ir, r \neq q}$ and $\mathbf{W}_{jp}$ for all $j < i$ and $p \in \{1 , \ldots , n_j\}$ where $n_j$ is the number of paragraphs in document $j$.
Likewise, $\mathbf{D}^{train}$ be the set of $\mathbf{D}_{ir, r \neq q}$ and $\mathbf{D}_{jp}$ for all $j < i$ and $p \in \{1 , \ldots , n_j\}$.

\begin{equation}
\begin{split}
  &p(\mathbf{W}_{iq}, \mathbf{D}_{iq} \vert \mathbf{W}^{train}, \mathbf{D}^{train}) \\
  &\propto \int_{\eta, \Psi, \tau} \sum_{\mathbf{Z}} p(\mathbf{W}_{iq}, \mathbf{D}_{iq} \vert \mathbf{Z}, \eta, \Psi, \tau) 
  \times p(\mathbf{Z}, \eta, \Psi, \tau, \vert \mathbf{W}^{train}, \mathbf{D}^{train}) d\eta d\Psi d\tau \\
  &\propto \int_{\eta, \Psi, \tau} \sum_{\mathbf{Z}} p(\mathbf{W}_{iq}, \mathbf{D}_{iq} \vert \mathbf{Z}, \eta, \Psi, \tau) 
  \times p(\mathbf{Z} \vert \eta, \Psi, \tau, \mathbf{W}^{train}, \mathbf{D}^{train}) p( \eta, \Psi, \tau \vert \mathbf{W}^{train}, \mathbf{D}^{train}) d\eta d\Psi d\tau \\
  &\approx \sum_{Z_{iq}} p(\mathbf{W}_{iq}, \mathbf{D}_{iq} \vert Z_{iq}, \hat{\mathbf{Z}}^{train}, \hat{\eta}, \hat{\Psi}, \hat{\tau}) \times p(Z_{iq} \vert \hat{\eta})  \\
  &= \sum_{k=1}^K \Big\{ p(\mathbf{W}_{iq}, \mathbf{D}_{iq} \vert Z_{iq} = k, \hat{\mathbf{Z}}^{train}, \hat{\eta}, \hat{\Psi}, \hat{\tau}) \times p(Z_{iq} = k \vert \hat{\eta}) \Big\} \\
  &= \sum_{k=1}^K \Big\{ p(\mathbf{W}_{iq} \vert Z_{iq} = k, \hat{\Psi})
  \times \prod_{j=1}^{i-1} p(D_{iqj} \vert \hat{\tau}, \hat{\eta}, Z_{ip})
  \times p(Z_{iq} = k \vert \hat{\eta}) \Big\} \\
  &= \sum_{k=1}^K \Big\{ p(\mathbf{W}_{iq} \vert Z_{iq} = k, \hat{\Psi})
  \times \prod_{j=1}^{i-1} \mathbb{P}(D_{iqj}^* > 0 \vert \hat{\tau}, \hat{\eta}, Z_{ip} = k)^{\mathbb{I}\{D_{iqj}=1\}}\mathbb{P}(D_{iqj}^* < 0 \vert \hat{\tau}, \hat{\eta}, Z_{ip} = k)^{\mathbb{I}\{D_{iqj}=0\}} \\
  &\quad \times p(Z_{iq} = k \vert \hat{\eta}) \Big\} \\
  &\propto \sum_{k=1}^K \Bigg\{ \prod_{v=1}^V \Psi_{vk}^{W_{iqv}} 
  \times \prod_{j=1}^{i-1} \Big[\int_{t=0}^{\infty} p(D_{iqj}^* = t | \tau_0 + \tau_1 \kappa_j^{(i)} + \tau_2\eta_{jk}) dt\Big]^{\mathbb{I}\{D_{iqj}=1\}} \\
  &\quad \times \Big[\int_{t=-\infty}^{0} p(D_{iqj}^* = t | \tau_0 + \tau_1 \kappa_j^{(i)} + \tau_2\eta_{jk}) dt \Big]^{\mathbb{I}\{D_{iqj}=0\}} 
  \times \frac{\exp(\eta_{ik})}{\sum_{k'=1}^K \exp(\eta_{ik'})} \Bigg\} \\
\end{split}
\end{equation}

The approximation part can use Monte Carlo simulation - We draw parameters $\eta, \tau$ from the posterior distributions and take the average.
Alternatively, we could use the point estimate of $\eta, \tau$ to match the computation in RTM and LDA+logistic.

